Mitigating spectral bias for the multiscale operator learning

Neural operators have emerged as a powerful tool for learning the mapping between infinite-dimensional parameter and solution spaces of partial differential equations (PDEs). In this work, we focus on multiscale PDEs that have important applications such as reservoir modeling and turbulence prediction. We demonstrate that for such PDEs, the spectral bias towards low-frequency components presents a significant challenge for existing neural operators. To address this challenge, we propose a hierarchical attention neural operator (HANO) inspired by the hierarchical matrix approach. HANO features a scale-adaptive interaction range and self-attentions over a hierarchy of levels, enabling nested feature computation with controllable linear cost and encoding/decoding of multiscale solution space. We also incorporate an empirical $H^1$ loss function to enhance the learning of high-frequency components. Our numerical experiments demonstrate that HANO outperforms state-of-the-art (SOTA) methods for representative multiscale problems.

==> Neurips2023/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,amssymb,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak
% comments
\newcommand{\xl}[1]{{\color{blue}#1}}
\newcommand{\lz}[1]{{\color{red}#1}}

==> figures/app.tex <==
%!TEX root = ../iclr2021\_conference.tex

\section{Transformer}

\lz{give some basics} 

Despite the enhanced expressibility, transformer models may suffer from the computational cost quadratically scaled with respect to the input, such as the resolution of images or parameters of the physical systems. Many tricks used in computational mathematics can be leveraged to alleviate the computation cost arising in dense matrix operation. Several recent works \cite{kitaev2020reformer,peng2021random,cao2021choose}  design transformers with near-linear complexity by exploiting the low rank structure of the dense attention matrix. But all these works trade accuracy for efficiency by dropping some local and detailed information. 

Both CNN and transformer utilize embedding to map discrete variables to high dimensional spaces. Interestingly, for multiscale PDE, analogous approaches have been developed to map low dimensional multiscale PDEs to high dimensional space.

Once the embedding mapping is done, the next task is to find the interaction between high dimensional vectors, for the PDE case, that will be a combination of the coefficient and solution. Transformer provides such utility but only at large scale, to further provide interaction of scales, we use a hierarchical structure to decompose the interaction between each subdomain at different scales. 

On the other hand, we plan to treat the PDE operator learning tasks with transformer models. FNO, ... \lz{to add} or operator learning for multiscale problems. 

So we plan to design a hierarchical transformer by introducing the most successful linear scaling numerical methods like multigrid method and hierarchical matrix. Models with Hierarchical  architecture \cite{he2019mgnet,liu2021swin} have already been applied to imagine classification successfully, which is a base of our extension to dense prediction task, including but not limited to neural operator learning and image segmentation. We believe the hierarchical transformer can keep both the fine and coarse details within near-linear computational costs by computing the attention matrix in a hierarchical fashion.


\begin{itemize}
    \item connection of high dimensional embedding to the mapping from multiscale PDE to high dimensional PDE
    \item sequential operation of MSA and FNO (convolution)
    \item  use MSA as a way to do high dimensional embedding for FNO
    \item to capture the fine scale feature, use hierarchical structure to reduce $O(N^2)$ cost of MSA to $O(N\log N)$
\end{itemize}


%----------------------------------
\section{Multiscale PDE}
\label{sec:msellipticpde}
%----------------------------------

%----------------------------------
\subsection{Homogenization}
\label{sec:msellipticpde:homognenization}
%----------------------------------

Suppose that $a^\varepsilon(x)$ in \eqref{eqn:darcy} takes a special form $a(\frac{x}{\varepsilon})$
  \begin{equation*}
    \left\{
      \begin{array}{lr}
        -\text{div} \left(a\left(\frac{x}{\varepsilon}\right)\nabla u^\varepsilon\right)=g & x\in\Omega \subset \R^d, a(\cdot) \text{  periodic \ in} \ y=x/\varepsilon, \\
        u^\varepsilon = 0 & x\in\partial\Omega \\
      \end{array}
    \right.
  \end{equation*}
  

  $u^\varepsilon \rightharpoonup u_0$ in $H^1$;  $u_0(x)$--coarse scale only, solves 
  the homogenized problem
  % 
  \begin{equation}
    \label{homogproblem}
    \left\{
      \begin{array}{lr}
	-\text{div}_x(\hat{a}\nabla_x u_0) = g & x\in\Omega \\
	u_0=0 & x\in\partial\Omega. \\
      \end{array}
    \right.
  \end{equation}
  

  $u^\varepsilon$--two scales, asymptotic expansion of $u^\varepsilon=u(x,x/\varepsilon)$ in $\varepsilon$ \\
  $\Rightarrow$ $d$ cell problems ($Y$--periodicity cell, $d$ dimension):
  
    \begin{equation*}
      \left\{
        \begin{array}{lr}
          -\text{div}_y \left(a\left(\nabla_y \chi_i+e_i\right)\right)=0 & x\in Y \text{, } 1\leq i \leq d \\
          \chi_i \in H^1_{\text{per}}(Y) \\
        \end{array}
      \right.
    \end{equation*}

  Two objectives: \\

  $\bullet$ Find effective coefficients  $\hat a$.
  

  Determined by cell problems only, $\hat{a}_{ij}=\int_Y (e_i+\nabla\chi_i)^T a(y) (e_j+\nabla \chi_j) dy$
  -- bypass for arbitrary coefficients.


  $\bullet$ Find approximate solution $\hat{u}^\varepsilon$--homogenization approximation.
  %
  \begin{equation*}
  \|u^\varepsilon - \hat{u}^\varepsilon\|_{H^1}\leq c \varepsilon^{\frac{1}{2}}, \text{where}
  \end{equation*}

  \begin{equation*}
  \begin{array}{rl}
  \hat{u}^\varepsilon &= u_0 -\varepsilon \sum \chi_i \left(\frac{x}{\varepsilon}\right) \frac{\partial u_0}{\partial x_i}
  %+\varepsilon^2\sum \theta^{kl}\left(\frac{x}{\varepsilon}\right) \frac{\partial^2 u_0}{\partial x_k\partial x_l}
  \\
  &=u_0+\varepsilon u_1%+\varepsilon^2 u_2
  \\
  \end{array}
  \end{equation*}

  $\chi_i$ are solutions of cell problems.  
  To find approximation $u_0$ (and $u_0+\varepsilon u_1$),
  solve coarse scale problem--requires precomputing $d$ cell problems for $\chi_i$ which do not depend on $g$ and $\Omega$.



\paragraph{Sobolev norm}
For $d \geq 1, \Omega$ an open subset of $\mathbb{R}^d,$ the Sobolev space $H^{1}\left(\mathbb{R}^d\right)$ is defined by $H^{1}(\Omega)=\left\{f \in L^2(\Omega):  \partial_{x_i} f \in L^2(\Omega),\, for, i = 1 \cdots d\right\}$ and the derivatives $\partial_{x_i} f$ are taken in a weak sense.
When endowed with the norm
$$
\|f\|_{1, \Omega}=\|f\|_{L^2(\Omega)}\sum_{i=1}^{n} \left\|\partial_{x_i} f\right\|_{L^2(\Omega)},
$$
$H^{1}(\Omega)$ is a Banach space.
\label{sec:multiscale PDE}
It is known that the solution space of the elliptic problem has the following Kolmogorov N-width in the sense that the best $N-$term approximation error of $V$ in terms of $\|\cdot\|_{H^1}$ norm, namely the \emph{Kolmogorov $N$ width}, $\sim N^{-1/d}\sim H$, due to the \emph{Compactness of the solution space} $V$   solution space $V:=\{u\in H^1_0(\Omega)| \nabla \cdot (a\nabla u)\in L^2(\Omega)\}$ is isomorphic to $H^2(\Omega)$ by the map $u' = \Delta^{-1} \nabla(a\nabla u)$. 


%----------------------------------
\subsection{Numerical Homogenization}
\label{sec:msellipticpde:numericalhomogenization}
%----------------------------------

In the context of PDEs governed operator learning, the above encoder decoder architecture share the same spirit with homogenization theory.
\xl{Effective coefficients is easy to illustrate.  }Review homogenized model, rethinking our model as discovering effective coefficients. Our model consists of two main parts. The multiscale coefficients are feed to a  hierarchical attention based encoder, and then passed to a Fourier spectral decoder to project the effective coefficients (encoded latent variable) to solution space. 

\xl{Introduce the homogenized model, which is a quasi local model. }
Let $V_{H}$ be the piecewise linear space defined on coarse triangle partition $T_H$. Define a quasi-local bilinear form,
$$\mathfrak{a}^{(\ell)}\left(v_{H}, z_{H}\right):=\int_{\Omega} \int_{\Omega} \nabla v_{H}(y) \cdot\left(\mathcal{A}_{H}^{(\ell)}(x, y) \nabla z_{H}(x)\right) d y d x \quad$$ for any $v_{H}, z_{H} \in V_{H}$.

We seek to solve the quasi-local model,
$$
\mathfrak{a}^{(\ell)}\left(u_{H}^{(\ell)}, v_{H}\right)=F\left(v_{H}\right).
$$

\subsection{Multilevel/multigrid method}


\subsection{Periodic unfolding}

\xl{Explain why Homogenized model better}




\section{Approximation Theory of Operator Learning}

\xl{Moved to Appendix if conference or can be left for Gamblets Framelets Operator Learning work}
\begin{itemize}
    \item Review the argument regarding universal approximation theory of general operator learning defined on Banach spaces\cite{kovachki2021universal}. Three key ingredients are compactness of the preimage set $K$, continuity of operator and the Schauder basis. \xl{We need verify the three key ingredients for the multiscale coefficients to solution map}
\end{itemize}


\begin{theorem}
    Let $s, s^{\prime} \geq 0$ and $\Omega \subset[0,2 \pi]^{d}$ be a domain with Lipschitz boundary. Let $\mathcal{G}: H^{s}\left(\Omega ; \mathbb{R}^{d_{a}}\right) \rightarrow H^{s^{\prime}}\left(\Omega ; \mathbb{R}^{d_{u}}\right)$ be a continuous operator. Let $K \subset$ $H^{s}\left(\Omega ; \mathbb{R}^{d_{a}}\right)$ be a compact subset. Then there exists a continuous, linear operator

$\mathcal{E}: H^{s}\left(\Omega ; \mathbb{R}^{d_{a}}\right) \rightarrow H^{s}\left(\mathbb{T}^{d} ; \mathbb{R}^{d_{a}}\right)$ such that $\left.\mathcal{E}(a)\right|_{\Omega}=a$ for all $a \in H^{s}\left(\Omega ; \mathbb{R}^{d_{a}}\right)$. Furthermore, for any $\epsilon>0$, there exists a FNO $\mathcal{N}: H^{s}\left(\mathbb{T}^{d} ; \mathbb{R}^{d_{a}}\right) \rightarrow H^{s^{\prime}}\left(\mathbb{T}^{d} ; \mathbb{R}^{d_{u}}\right)$ of the form (2.6), such that
$$
\sup _{a \in K}\left\|\mathcal{G}(a)-\left.\mathcal{N} \circ \mathcal{E}(a)\right|_{\Omega}\right\|_{H^{s^{\prime}}} \leq \epsilon .
$$
\end{theorem}

\begin{itemize}
    \item \xl{Review the theory that the coefficient to solution mapping is differentiable. This is not clear in paper \cite{kovachki2021universal}}. Clarify what is missing there, for Darcy in specific. Their restriction on $H^s$ space and so on. This part could be left to more comprehensive version.
\end{itemize}
We study the mapping   $\mathcal{N}:K=\left\{\kappa \in L^\infty (D;\mathbb{R}_+): k_{0} \leq \kappa \leq k_{1}\right\} \rightarrow H_0^1(D;\mathbb{R})$ such that $a \mapsto \mathcal{N}(a):= u$, where $u$ is the solution to \eqref{eqn:darcy}.
 
 
We write $V=H_{0}^{1}(\Omega), B=L^{\infty}(\Omega)$, and define $T: K \times V \times V \rightarrow \mathbb{R}$ by
$$
T(\kappa, u, v)=\int_{\Omega} \kappa \nabla u \cdot \nabla v .
 $$
% The trilinear form $T$ then satisfies the conditions
% $$
% \begin{aligned}
% &T(q, u, v) \leq \beta\|q\|_{B}\|u\|_{V}\|v\|_{V} \text { for all } u, v \in V, q \in B \\
% &T(q, u, u) \geq \alpha\|u\|_{V}^{2} \text { for all } u \in V, q \in A
% \end{aligned}
% $$
% where $A=\left\{q \in L^{\infty}(\Omega): k_{0} \leq q \leq k_{1}\right\}, \beta=1$ and $\alpha>0$ comes from Poincaré's inequality.
\begin{theorem}
    The operator $\mathcal{N}$ is continuous and
$$
\|\mathcal{N}(\kappa)-\mathcal{N}(\kappa')\|_{V} \leq \frac{k_1}{k_0} \min \left\{\|\mathcal{N}(\kappa)\|_{V},\|\mathcal{N}(\kappa')\|_{V}, \frac{\|f\|_{V^{*}}}{k_0}\right\}\|\kappa-\kappa'\|_{B}
$$
\end{theorem} 
\begin{theorem}
    For each $\kappa$ in the interior of $K$, $\mathcal{N}$ is differentiable at $\kappa$, and $\delta u=D \mathcal{N}(\kappa) \delta \kappa$ is the unique solution to the variational equation
$$
T(a, \delta u, v)=-T(\delta a, u, v) \text { for all } v \in V,
$$
where $u=F(a)$. Moreover,
$$
\|D F(a)\| \leq \frac{\beta}{\alpha}\|F(a)\|_{V} \leq \frac{\beta}{\alpha^{2}}\|m\|_{V^{*}} .
$$
\end{theorem}

\section{Neural Operator Architecture and Implementation Details}
\label{sec:implementation}

\paragraph{Patch Embedding}
\paragraph{Position Embedding}
\begin{remark}
In the implementation of Darcy flow operator learning, their input is the function $\hat{a}: D\rightarrow \mathbb{R}^3$. $\hat{a}(x) = (a(x), x_1, x_2) \in \mathbb{R}^3$ is the  concatenation of diffusion coefficient and the coordinates. In that case, $P\in \mathbb{R}^{d_v\times 3}$.
\end{remark}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.7\textwidth]{darcySol_eigen.png}
    \caption{Eigenvalues distribution for different data sets.}
    \label{fig:eigen_dist}
\end{figure}
 
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.7\textwidth]{figures/liftingOperator.JPG}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}



\section{Approximation error from H matrix perspective}
The key idea of the FMM is to approximate interacting function $\mathcal{G}$ in \eqref{eqn:Green's} restricted on well separated boxes by a truncated series expansion. For $x, x'$ located in well separated cubes $c$ and  $c^{\prime}$, respectively.  
\begin{equation}
    \mathcal{G}(\boldsymbol{x}, \boldsymbol{x'})\approx  \sum_{|\alpha| \leq p|\beta| \leq p-|\alpha|} \frac{D^{\alpha+\beta} \mathcal{G}\left(\left|r_{c c^{\prime}}\right|\right)}{\alpha ! \beta !}\left(\boldsymbol{x}-\boldsymbol{x}_{c}\right)^{\alpha} \left(\boldsymbol{x}_{c^{\prime}}-\boldsymbol{x}^{\prime}\right)^{\beta},
\end{equation}
where $r_{c c^{\prime}}=\|\boldsymbol{x}_{c}-\boldsymbol{x}_{c^{\prime}}\|$ is the distance between the average center of the particles located in the separated cubes and $p$ be the expansion order. 

use neighbor in geometry space, to approximate neighbors in feature space, 
\paragraph{the benifits of hierarchical attention} implicit and balanced position embedding, 


Let $\varphi_{c, c^{\prime}}$ be the potential evaluated in the well separated cube $c$, due to particles in cube $c^{\prime}$, then
$$
\begin{aligned}
\varphi_{c c^{\prime}}(\boldsymbol{x}) &=\int_{S_{c^{\prime}}} \mathcal{G}\left(\left|\boldsymbol{x}-\boldsymbol{x}^{\prime}\right|\right) v\left(\boldsymbol{x}^{\prime}\right) d s\left(\boldsymbol{x}^{\prime}\right) \\
& \approx \sum_{|\alpha| \leq p|\beta| \leq p-|\alpha|} \frac{D^{\alpha+\beta} \mathcal{G}\left(\left|r_{c c^{\prime}}\right|\right)}{\alpha ! \beta !}\left(\boldsymbol{x}-\boldsymbol{x}_{c}\right)^{\alpha} \int_{S_{c}^{\prime}}\left(\boldsymbol{x}_{c^{\prime}}-\boldsymbol{x}^{\prime}\right)^{\beta} v\left(\boldsymbol{x}^{\prime}\right) d s\left(\boldsymbol{x}^{\prime}\right) \\
&=\sum_{|\alpha| \leq p} \lambda_{c, c^{\prime}}^{\alpha}\left(\boldsymbol{x}-\boldsymbol{x}_{c}\right)^{\alpha}, \quad \boldsymbol{x} \in S_{c}
\end{aligned}
$$
where $\alpha, \beta$ are multiindices . Here the local expansion coefficient $\lambda_{c, c^{\prime}}^{\alpha}$ is given by
$$
\lambda_{c, c^{\prime}}^{\alpha}=\sum_{|\beta| \leq p-|\alpha|} \frac{D^{\alpha+\beta} \mathcal{G}\left(\left|r_{c c^{\prime}}\right|\right)}{\alpha ! \beta !}(-1)^{|\beta|} m_{c^{\prime}}^{\beta}(v), \quad|\alpha| \leq p
$$
where $m_{v^{\prime}}^{\beta}(v)$ is a moment of the function $v$, which is given by
$$
m_{v^{\prime}}^{\beta}(v)=\int_{S_{v^{\prime}}} \left(x-x_{v^{\prime}}\right)^{\beta} v(\boldsymbol{x}) d s(\boldsymbol{x}), \quad|\beta| \leq p
$$

\section{Data Sampling}


\subparagraph{KL expansion}
In the context of operator learning, the input $u(t)$ is sampled from a stochastic Gaussian process with a specified covariance function.
We will consider a square-integrable zero-mean Gaussian process $X_{t}$ defined over a probability space $(\Omega, F, \mathbf{P})$   and indexed over a closed interval $[a, b] $ , with covariance function  $K_{X}(s, t)$.   

We thus have $\forall t \in[a, b]$, $X_{t} \in L^{2}(\Omega, F, \mathbf{P})$,  $\mathbf{E}\left[X_{t}\right]=0.$ 
$ K_{X}(s, t)=\mathbf{E}\left[X_{s} X_{t}\right],\, \forall t, s \in[a, b].$  
We associate to $K_{X}$ a  linear operator $T_{K_{X}}$  defined in the following way:
$$
\begin{aligned}
T_{K_X}: L^2([a,b]) &\to  L^2([a,b])\\
: f \mapsto T_{K_X}f &= \int_a^b K_X(s,\cdot) f(s) \, ds
\end{aligned}
$$
Since $T_{X_{X}}$  is a linear operator, it makes sense to talk about its eigenvalues $\lambda_{k} $ and eigenfunctions $ e_{k}$, which are found solving the homogeneous Fredholm integral equation of the second kind $ \int_{a}^{b} K_{X}(s, t) e_{k}(s) d s=\lambda_{k} e_{k}(t)$

\begin{theorem}[Karhunen-Loeve]
    Let $X_{t}$ be a zero-mean square-integrable stochastic process defined over a probability space $(\Omega, F, \mathbf{P})$ and indexed over a closed and bounded interval $[a, b]$, with continuous covariance function $K_{X}(s, t)$. Then $K_{X}(s, t)$ is a Mercer kernel and letting $e_{k}$ be an orthonormal basis on $L^{2}([a, b])$ formed by the eigenfunctions of $T_{K_{X}}$ with respective eigenvalues $\lambda_{k} X_{t}$ admits the following representation
    $$
    X_{t}=\sum_{k=1}^{\infty} Z_{k} e_{k}(t)
    $$
    where the convergence is in $L^{2}(\Omega)$, uniform in $t$ and
    $$
    Z_{k}=\int_{a}^{b} X_{t} e_{k}(t) d t
    $$
    Furthermore, the random variables $Z_{k}$ have zero-mean, are uncorrelated and have variance $\lambda_{k}$
    $$
    \mathbf{E}\left[Z_{k}\right]=0, \forall k \in \mathbb{N} \quad \text { and } \quad \mathbf{E}\left[Z_{i} Z_{j}\right]=\delta_{i j} \lambda_{j}, \forall i, j \in \mathbb{N}
    $$
    Let
    $$
    S_{N}=\sum_{k=1}^{N} Z_{k} e_{k}(t) .
    $$
    Then
    $$
    \mathbf{E}\left[\left|X_{t}-S_{N}\right|^{2}\right] \leq \sum_{i> k} \lambda_i^2,
    $$
    which means the approximation rate depends on how fast the eigenvalues decay.
\end{theorem}
% \begin{proof}
%     The covariance function $K_{X}$ satisfies the definition of a Mercer kernel. By Mercer's theorem, there consequently exists a set $\lambda_{k}, e_{k}(t)$ of eigenvalues and eigenfunctions of $\mathrm{T}_{K_{X}}$ forming an orthonormal basis of $L^{2}([a, b])$, and $K_{X}$ can be expressed as
% $$
% K_{X}(s, t)=\sum_{k=1}^{\infty} \lambda_{k} e_{k}(s) e_{k}(t)
% $$
% The process $X_{t}$ can be expanded in terms of the eigenfunctions $e_{k}$ as:
% $$
% X_{t}=\sum_{k=1}^{\infty} Z_{k} e_{k}(t)
% $$
% where the coefficients (random variables) $Z_{k}$ are given by the projection of $X_{t}$ on the respective eigenfunctions
% $$
% Z_{k}=\int_{a}^{b} X_{t} e_{k}(t) d t
% $$
% We may then derive
% $$
% \begin{aligned}
% \mathbf{E}\left[Z_{k}\right] &=\mathbf{E}\left[\int_{a}^{b} X_{t} e_{k}(t) d t\right]=\int_{a}^{b} \mathbf{E}\left[X_{t}\right] e_{k}(t) d t=0 \\
% \mathbf{E}\left[Z_{i} Z_{j}\right] &=\mathbf{E}\left[\int_{a}^{b} \int_{a}^{b} X_{t} X_{s} e_{j}(t) e_{i}(s) d t d s\right] \\
% &=\int_{a}^{b} \int_{a}^{b} \mathbf{E}\left[X_{t} X_{s}\right] e_{j}(t) e_{i}(s) d t d s \\
% &=\int_{a}^{b} \int_{a}^{b} K_{X}(s, t) e_{j}(t) e_{i}(s) d t d s \\
% &=\int_{a}^{b} e_{i}(s)\left(\int_{a}^{b} K_{X}(s, t) e_{j}(t) d t\right) d s \\
% &=\lambda_{j} \int_{a}^{b} e_{i}(s) e_{j}(s) d s \\
% &=\delta_{i j} \lambda_{j}
% \end{aligned}
% $$
% where we have used the fact that the $e_{k}$ are eigenfunctions of $T_{K_{X}}$ and are orthonormal.

% Let us now show that the convergence is in $L^{2}$. Let
% $$
% S_{N}=\sum_{k=1}^{N} Z_{k} e_{k}(t) .
% $$
% Then
% $$
% \begin{aligned}
% \mathbf{E}\left[\left|X_{t}-S_{N}\right|^{2}\right] &=\mathbf{E}\left[X_{t}^{2}\right]+\mathbf{E}\left[S_{N}^{2}\right]-2 \mathbf{E}\left[X_{t} S_{N}\right] \\
% &=K_{X}(t, t)+\mathbf{E}\left[\sum_{k=1}^{N} \sum_{l=1}^{N} Z_{k} Z_{\ell} e_{k}(t) e_{\ell}(t)\right]-2 \mathbf{E}\left[X_{t} \sum_{k=1}^{N} Z_{k} e_{k}(t)\right] \\
% &=K_{X}(t, t)+\sum_{k=1}^{N} \lambda_{k} e_{k}(t)^{2}-2 \mathbf{E}\left[\sum_{k=1}^{N} \int_{a}^{b} X_{t} X_{s} e_{k}(s) e_{k}(t) d s\right] \\
% &=K_{X}(t, t)-\sum_{k=1}^{N} \lambda_{k} e_{k}(t)^{2}
% \end{aligned}
% $$
% which goes to 0 by Mercer's theorem.
% \end{proof}

% Associated to $K$ is a linear operator (more specifically a Hilbert-Schmidt integral operator) on functions defined by the integral
% $$
% \left[T_{K} \varphi\right](x)=\int_{a}^{b} K(x, s) \varphi(s) d s .
% $$
% For technical considerations we assume $\varphi$ can range through the space $L^{2}[a, b]$ (see $L p$ space) of square-integrable real-valued functions. Since $T_{K}$ is a linear operator, we can talk about eigenvalues and eigenfunctions of $T_{K}$.
\begin{theorem}[General Mercer's Theorem ]
    Suppose $K$ is a continuous symmetric non-negative definite kernel. Then there is an orthonormal basis $\{e_i\}$  of $L^{2}\left[a_{i} b\right]$ consisting of eigenfunctions of $T_{K}$ such that the corresponding sequence of eigenvalues $\{\lambda_{j} \}$ is nonnegative. The eigenfunctions corresponding to non-zero eigenvalues are continuous on $[a, b]$ and $K$ has the representation
$$
K(s, t)=\sum_{j=1}^{\infty} \lambda_{j} e_{j}(s) e_{j}(t)
$$
where the convergence is absolute and uniform.
\end{theorem} 

By KL expansion, we only need to sample Gaussian variables $Z_k\sim \mathcal{N}(0, \lambda_k)$, and recover the samples by the truncated formula 
$$
S_{N}=\sum_{k=1}^{N} Z_{k} e_{k}(t) .
$$.
% \begin{Theorem}[Mercer's Theorem]
% 	Let $(\mathcal{X}, \mu)$ be a finite measure space and $K \in L_{\infty}\left(\mathcal{X}^{2}, \mu^{2}\right)$ be a kernel such that $T_{K}: L_{2}(\mathcal{X}, \mu) \rightarrow L_{2}(\mathcal{X}, \mu)$ is positive definite. Let $\phi_{i} \in L_{2}(\mathcal{X}, \mu)$ be the normalized eigenfunctions of $T_{K}$ associated with the eigenvalues $\lambda_{i}>0$. Then
% 	$$
% 	K\left(\mathbf{x}, \mathbf{x}^{\prime}\right)=\sum_{i=1}^{\infty} \lambda_{i} \phi_{i}(\mathbf{x}) \phi_{i}^{*}\left(\mathbf{x}^{\prime}\right)
% 	$$
% 	holds $\mu^{2}$ almost everywhere, where the series converges absolutely and uniformly $\mu^{2}$ almost everywhere.
% \end{Theorem}
\subparagraph{KL expansion for Laplacian related kernel}
In the case of FNO's examples, the coefficients $a\in L^{\infty}([0, 2\pi]),\ a(x)\geq a_{\min} >0$ are generated by 2 steps. 

Step1. Pre-coefficients $\hat{a}$  are sampled from a centered Gaussian process $X_t \sim \mathcal{G P}\left(0, -\Delta+9 I)^{-2} \right)$, with specific covariance function  $(-\Delta+9 I)^{-2}$, where $\Delta$ is defined on $[0, 2\pi]$ with zero Neumann boundary conditions. Then,
$$
\begin{aligned}
T_{K_X}: L^2([0, 2\pi]) &\to  L^2([0, 2\pi])\\
: f \mapsto T_{K_X}f &= \int_0^2\pi \left(0,(-\Delta+9 I)^{-2}\right) f(s) \, ds.
\end{aligned}
$$
One can find the eigenfunctions and eigenvalues of $T_{K_X}$ are
$$
\begin{gathered}
\lambda_{k}= (i^2+9)^{-2}, \quad k=0,1,2, \ldots, \\
e_{k}(x)= cos(kx) .
\end{gathered}
$$
In practise, the truncated formula 
$$
S_{N}=\sum_{k=1}^{N} Z_{k} e_{k}(t) .
$$
allow us  to sample efficiently and accurately.

Step2. We further apply a nonlinear mapping $\psi$  on $\hat{a}$ to impose the elliptic constrains.  The mapping $\psi: \mathbb{R} \rightarrow \mathbb{R}$ takes the value 12 on the positive part of the real line and 2 on the negative and the operation is defined pointwisely.
$
a = \psi(\hat{a})
$ is a piecewise constant function on $[0,  2\pi]$.

% \section{figure}
% \begin{figure}[H]
%     \centering
%     \includegraphics[width=.7\textwidth]{figures/archi.jpg}
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}

